LOLA -- An Open-Source Massively Multilingual Large Language Model

This paper presents LOLA, a massively multilingual large language model trained on more than 160 languages using a sparse Mixture-of-Experts Transformer architecture. Our architectural and implementation choices address the challenge of harnessing linguistic diversity while maintaining efficiency and avoiding the common pitfalls of multilinguality. Our analysis of the evaluation results shows competitive performance in natural language generation and understanding tasks. Additionally, we demonstrate how the learned expert-routing mechanism exploits implicit phylogenetic linguistic patterns to potentially alleviate the curse of multilinguality. We provide an in-depth look at the training process, an analysis of the datasets, and a balanced exploration of the model's strengths and limitations. As an open-source model, LOLA promotes reproducibility and serves as a robust foundation for future research. Our findings enable the development of compute-efficient multilingual models with strong, scalable performance across languages.

==> tables/arc.tex <==
%\documentclass[11pt, a4paper]{article}
%\usepackage{booktabs}
%\begin{document}

\begin{table*}[htb]
    \centering
    \caption{Arc task}
    \label{tab:arc}
    \resizebox{1.9\columnwidth}{!}{%
    \begin{tabular}{@{}lcccccccc@{}}
    \hline
        \toprule
        Language & lola\_v1 &xlm-roberta-large & mGPT & bloom-1b1 & bloom-1b7 & glot500-base & mbart-large-50 & mt5-large 
         \\
        \midrule
        ar & 22.24 & 23.1 & 20.36 & 21.13 & 21.73 & 23.1 & 20.96 & 20.36 \\ 
        bn & 18.91 & 20.27 & 18.91 & 19.5 & 21.04 & 20.79 & 20.19 & 20.19 \\
        ca & 23.84 & 23.33 & 18.87 & 22.56 & 21.96 & 21.87 & 20.33 & 22.3 \\
        da & 21.85 & 22.19 & 19.45 & 19.97 & 19.37 & 20.14 & 18.77 & 21.42 \\
        de & 23.44 & 20.79 & 18.99 & 20.79 & 19.93 & 18.91 & 20.19 & 20.27 \\
        es & 24.53 & 21.28 & 19.4 & 23.08 & 22.99 & 20.77 & 19.91 & 21.03 \\
        eu & 21.79 & 22.58 & 20.83 & 21.62 & 22.14 & 21.53 & 21.7 & 20.83 \\
        fr & 23.1 & 22.75 & 20.19 & 21.98 & 23.52 & 22.5 & 20.7 & 21.56 \\
        gu & 21.81 & 22.16 & 22.24 & 22.07 & 21.47 & 22.24 & 20.86 & 22.41 \\
        hi & 20.89 & 21.83 & 19.86 & 21.23 & 19.95 & 22.35 & 19.26 & 21.92 \\
        hr & 19.67 & 22.24 & 18.91 & 19.59 & 18.22 & 22.58 & 20.53 & 21.73 \\
        hu & 22.43 & 17.89 & 19.09 & 18.84 & 19.86 & 18.75 & 19.86 & 19.78 \\
        hy & 22.36 & 24.18 & 21.82 & 21.09 & 22.82 & 23.91 & 21.18 & 21.73 \\
        id & 20.51 & 20.77 & 17.95 & 20.09 & 20.77 & 21.03 & 19.74 & 19.06 \\
        it & 24.81 & 21.04 & 20.27 & 19.67 & 20.27 & 19.93 & 20.1 & 20.62 \\
        kn & 20.3 & 21.43 & 20.47 & 20.38 & 20.64 & 21.34 & 20.12 & 20.73 \\
        ml & 22.24 & 23.64 & 21.54 & 21.37 & 21.54 & 22.59 & 21.54 & 21.63 \\
        mr & 22.34 & 24.59 & 22.34 & 22.86 & 22.34 & 23.2 & 22.51 & 21.13 \\
        ne & 19.42 & 21.3 & 22.16 & 21.21 & 20.27 & 22.75 & 20.53 & 22.5 \\
        nl & 21.21 & 20.36 & 19.76 & 18.82 & 19.25 & 19.76 & 21.56 & 19.25 \\
        pt & 25.04 & 22.05 & 21.03 & 24.1 & 23.59 & 21.62 & 21.62 & 22.65 \\
        ro & 23.65 & 19.97 & 20.22 & 18.85 & 18.94 & 20.48 & 18.85 & 19.45 \\
        ru & 23.35 & 21.13 & 20.19 & 19.59 & 19.25 & 21.13 & 21.04 & 20.19 \\
        sk & 23.95 & 20.02 & 18.48 & 18.39 & 18.31 & 20.27 & 19.93 & 21.47 \\
        sr & 20.36 & 22.24 & 17.45 & 18.82 & 16.77 & 21.56 & 19.5 & 21.39 \\
        sv & 23.26 & 20.34 & 20.43 & 19.66 & 19.4 & 20.09 & 21.89 & 19.4 \\
        ta & 22.33 & 20.23 & 21.37 & 23.38 & 21.89 & 19.53 & 22.85 & 21.02 \\
        te & 19.21 & 22.81 & 17.89 & 19.74 & 19.56 & 21.67 & 20.96 & 20.35 \\
        uk & 22.67 & 21.3 & 19.16 & 21.13 & 19.5 & 22.5 & 18.99 & 20.53 \\
        vi & 24.1 & 20.68 & 21.2 & 22.56 & 23.59 & 21.45 & 19.57 & 20.94 \\
        zh & 21.79 & 21.71 & 21.45 & 22.05 & 24.7 & 22.05 & 21.28 & 21.54 \\
        \bottomrule
    \end{tabular}
    }
\end{table*}

%\end{document}


==> tables/belebele.tex <==
%\documentclass[11pt, a4paper]{article}
%\usepackage{booktabs}
%\begin{document}

\begin{table*}[htb]
    \centering
    \caption{belebele task}
    \label{tab:belebele}
    \resizebox{1.9\columnwidth}{!}{%
    \begin{tabular}{@{}lcccccccc@{}}
    \hline
        \toprule
        Language & lola\_v1 &xlm-roberta-large & mGPT & bloom-1b1 & bloom-1b7 & glot500-base & mbart-large-50 & mt5-large 
         \\
        \midrule
        acm\_Arab & 24.22 & 23.67 & 23.0 & 22.89 & 23.22 & 22.33 & 27.33 & 22.89 \\
        afr\_Latn & 23.78 & 22.11 & 23.89 & 24.0 & 23.0 & 22.33 & 27.33 & 22.89 \\
        als\_Latn & 23.78 &  & 25.67 & 22.78 & 23.78 &  & 27.33 & 22.89 \\
        amh\_Ethi & 23.44 &  & 28.0 & 22.33 & 26.0 & 21.0 & 27.33 & 22.89 \\
        apc\_Arab & 24.44 & 24.22 & 23.22 & 23.44 & 22.89 & 20.67 & 27.33 & 22.89 \\
        arb\_Arab & 25.44 & 24.0 & 23.44 & 23.0 & 22.78 & 21.44 & 27.33 & 22.89 \\
        arb\_Latn & 23.33 &  & 23.56 & 24.44 & 24.22 &  & 27.33 & 22.89 \\
        ars\_Arab & 25.44 & 22.22 & 23.22 & 22.11 & 22.44 & 22.0 & 27.33 & 22.89 \\
        ary\_Arab & 24.11 &  & 24.44 & 21.44 & 22.78 & 23.0 & 27.33 & 22.89 \\
        arz\_Arab & 25.33 & 23.0 & 25.11 & 21.56 & 24.22 & 20.11 & 27.33 & 22.89 \\
        asm\_Beng & 24.44 &  & 24.89 & 27.11 & 27.0 &  & 27.33 & 22.89 \\
        azj\_Latn & 25.78 & 21.56 & 28.0 & 22.56 & 24.67 & 22.22 & 27.33 & 22.89 \\
        bam\_Latn & 23.44 &  & 26.44 & 22.11 & 22.56 & 21.67 & 27.33 & 22.89 \\
        ben\_Beng & 23.89 &  & 25.56 & 26.22 & 28.78 & 20.44 & 27.33 & 22.89 \\
        ben\_Latn & 26.22 &  & 25.33 & 23.0 & 25.44 &  & 27.33 & 22.89 \\
        bod\_Tibt & 22.78 & 22.67 & 20.11 & 28.89 & 22.33 &  & 27.33 & 22.89 \\
        bul\_Cyrl & 24.0 & 22.56 & 23.89 & 24.0 & 25.11 & 20.56 & 27.33 & 22.89 \\
        cat\_Latn & 24.78 & 22.33 & 23.67 & 25.78 & 24.44 & 22.11 & 27.33 & 22.89 \\
        ceb\_Latn & 26.0 &  & 23.22 & 22.78 & 23.22 & 24.11 & 27.33 & 22.89 \\
        ces\_Latn & 23.11 & 22.89 & 23.44 & 23.33 & 22.33 & 20.89 & 27.33 & 22.89 \\
        ckb\_Arab & 28.11 &  & 24.22 & 22.33 & 22.67 & 22.78 & 27.33 & 22.89 \\
        dan\_Latn & 24.67 & 21.11 & 24.11 & 25.44 & 23.56 & 20.44 & 27.33 & 22.89 \\
        deu\_Latn & 23.33 & 21.33 & 24.67 & 22.89 & 22.78 & 22.11 & 27.33 & 22.89 \\
        ell\_Grek & 25.67 &  & 23.33 & 22.89 & 22.89 &  & 27.33 & 22.89 \\
        eng\_Latn & 24.56 & 22.89 & 23.22 & 23.67 & 25.78 & 21.0 & 27.33 & 22.89 \\
        est\_Latn & 22.89 & 23.44 & 23.0 & 23.0 & 23.0 & 23.44 & 27.33 & 22.89 \\
        eus\_Latn & 24.67 & 22.89 & 26.67 & 23.78 & 23.89 & 23.22 & 27.33 & 22.89 \\
        fin\_Latn & 22.78 & 22.22 & 23.33 & 22.89 & 23.89 & 21.22 & 27.33 & 22.89 \\
        fra\_Latn & 24.33 &  & 24.44 & 22.22 & 23.33 & 20.78 & 27.33 & 22.89 \\
        fuv\_Latn & 22.78 &  & 22.78 & 21.56 & 22.78 & 23.0 & 27.33 & 22.89 \\
        gaz\_Latn & 23.56 &  & 23.67 & 22.0 & 22.89 &  & 27.33 & 22.89 \\
        grn\_Latn & 23.67 &  & 22.44 & 22.78 & 23.22 & 21.56 & 27.33 & 22.89 \\
        guj\_Gujr & 25.67 &  & 27.11 & 23.22 & 23.0 & 21.78 & 27.33 & 22.89 \\
        hat\_Latn & 22.89 &  & 24.44 & 24.11 & 23.22 & 22.0 & 27.33 & 22.89 \\
        hau\_Latn & 23.44 &  & 23.89 & 21.44 & 21.89 & 21.78 & 27.33 & 22.89 \\
        heb\_Hebr & 24.56 & 22.78 & 24.44 & 24.0 & 23.56 & 21.44 & 27.33 & 22.89 \\
        hin\_Deva & 26.89 & 21.67 & 26.11 & 28.11 & 23.11 & 21.67 & 27.33 & 22.89 \\
        hin\_Latn & 24.56 &  & 22.78 & 22.44 & 23.44 &  & 27.33 & 22.89 \\
        hrv\_Latn & 24.78 & 23.22 & 23.78 & 24.67 & 24.56 & 22.22 & 27.33 & 22.89 \\
        hun\_Latn & 24.56 & 22.78 & 23.0 & 25.33 & 23.11 & 20.67 & 27.33 & 22.89 \\
        hye\_Armn & 23.78 &  & 24.67 & 23.67 & 23.56 & 22.67 & 27.33 & 22.89 \\
        ibo\_Latn & 23.67 &  & 23.56 & 21.78 & 23.78 & 18.89 & 27.33 & 22.89 \\
        ilo\_Latn & 23.11 &  & 22.89 & 22.0 & 22.67 &  & 27.33 & 22.89 \\
        ind\_Latn & 23.78 & 23.44 & 23.0 & 22.44 & 22.89 & 20.11 & 27.33 & 22.89 \\
        isl\_Latn & 24.56 & 22.44 & 23.11 & 23.67 & 24.56 & 21.89 & 27.33 & 22.89 \\
        ita\_Latn & 24.33 & 22.33 & 24.0 & 21.44 & 23.11 & 21.56 & 27.33 & 22.89 \\
        jav\_Latn & 25.33 & 23.0 & 24.11 & 21.78 & 22.67 & 21.78 & 27.33 & 22.89 \\
        jpn\_Jpan & 24.56 & 21.67 & 24.89 & 25.67 & 25.44 & 21.33 & 27.33 & 22.89 \\
        kac\_Latn & 23.78 &  & 22.44 & 23.0 & 23.0 &  & 27.33 & 22.89 \\
        kan\_Knda & 24.11 &  & 21.89 & 23.67 & 23.78 &  & 27.33 & 22.89 \\
        kat\_Geor & 24.44 &  & 23.33 & 21.44 & 23.33 &  & 27.33 & 22.89 \\
        kaz\_Cyrl & 24.78 & 22.67 & 26.44 & 23.11 & 24.33 & 20.89 & 27.33 & 22.89 \\
        kea\_Latn & 24.44 &  & 22.0 & 23.0 & 23.44 & 21.67 & 27.33 & 22.89 \\
        khk\_Cyrl & 26.0 & 21.67 & 24.44 & 23.56 & 23.33 & 22.11 & 27.33 & 22.89 \\
        khm\_Khmr & 22.89 &  & 23.67 & 24.44 & 24.11 &  & 27.33 & 22.89 \\
        kin\_Latn & 27.22 &  & 26.44 & 23.11 & 24.44 &  & 27.33 & 22.89 \\
        kir\_Cyrl & 26.22 & 24.0 & 25.11 & 22.44 & 23.56 & 20.11 & 27.33 & 22.89 \\
        kor\_Hang & 25.44 & 24.0 & 23.56 & 28.67 & 22.67 & 21.44 & 27.33 & 22.89 \\
        lao\_Laoo & 22.89 &  & 23.44 & 21.89 & 22.56 &  & 27.33 & 22.89 \\
        lin\_Latn & 25.33 &  & 28.11 & 24.67 & 26.11 & 22.0 & 27.33 & 22.89 \\
        lit\_Latn & 24.11 & 23.22 & 23.67 & 21.33 & 24.11 & 22.11 & 27.33 & 22.89 \\
        lug\_Latn & 25.11 &  & 25.89 & 23.56 & 23.67 & 21.44 & 27.33 & 22.89 \\
        luo\_Latn & 23.67 &  & 23.33 & 24.89 & 24.33 & 20.22 & 27.33 & 22.89 \\
        lvs\_Latn & 24.22 & 22.11 & 26.89 & 23.33 & 24.11 & 22.67 & 27.33 & 22.89 \\
        mal\_Mlym & 24.0 &  & 24.44 & 28.22 & 23.33 &  & 27.33 & 22.89 \\
        mar\_Deva & 25.22 &  & 24.33 & 28.22 & 23.78 & 21.33 & 27.33 & 22.89 \\
        mkd\_Cyrl & 25.89 & 23.0 & 25.11 & 22.56 & 23.67 & 20.56 & 27.33 & 22.89 \\
        mlt\_Latn & 25.11 &  & 22.89 & 22.89 & 24.56 &  & 27.33 & 22.89 \\
        mri\_Latn & 23.33 &  & 23.0 & 22.89 & 22.89 &  & 27.33 & 22.89 \\
        mya\_Mymr & 25.56 &  & 24.33 & 23.67 & 23.0 &  & 27.33 & 22.89 \\
        nld\_Latn & 23.89 & 22.11 & 21.89 & 24.0 & 23.11 & 21.56 & 27.33 & 22.89 \\
        nob\_Latn & 23.11 & 22.44 & 25.11 & 25.67 & 23.44 & 20.67 & 27.33 & 22.89 \\
        npi\_Deva & 27.0 & 22.78 & 23.89 & 23.22 & 25.0 & 22.0 & 27.33 & 22.89 \\
        npi\_Latn & 25.11 &  & 22.78 & 22.89 & 23.22 & 23.0 & 27.33 & 22.89 \\
        nso\_Latn & 23.67 &  & 22.0 & 22.67 & 23.33 &  & 27.33 & 22.89 \\
        nya\_Latn & 24.11 &  & 22.89 & 22.11 & 22.89 & 21.33 & 27.33 & 22.89 \\
        ory\_Orya & 24.0 &  & 23.11 & 23.44 & 24.33 &  & 27.33 & 22.89 \\
        pan\_Guru & 23.67 &  & 23.78 & 26.67 & 23.22 &  & 27.33 & 22.89 \\
        pbt\_Arab & 23.67 &  & 21.44 & 21.11 & 23.78 &  & 27.33 & 22.89 \\
        pes\_Arab & 23.89 & 22.33 & 24.78 & 21.67 & 22.56 & 20.67 & 27.33 & 22.89 \\
        plt\_Latn & 22.89 &  & 23.0 & 22.67 & 24.33 &  & 27.33 & 22.89 \\
        pol\_Latn & 23.56 & 22.67 & 24.89 & 24.11 & 22.11 & 20.56 & 27.33 & 22.89 \\
        por\_Latn & 23.78 & 23.56 & 22.89 & 22.33 & 24.33 & 19.67 & 27.33 & 22.89 \\
        ron\_Latn & 23.33 & 22.22 & 22.78 & 23.0 & 23.11 & 23.0 & 27.33 & 22.89 \\
        rus\_Cyrl & 24.33 & 22.33 & 25.11 & 21.67 & 23.78 & 21.44 & 27.33 & 22.89 \\
        shn\_Mymr & 24.67 &  & 23.11 & 23.0 & 23.33 &  & 27.33 & 22.89 \\
        sin\_Latn & 23.56 &  & 22.22 & 22.78 & 22.67 &  & 27.33 & 22.89 \\
        sin\_Sinh & 23.67 &  & 22.89 & 22.78 & 23.44 &  & 27.33 & 22.89 \\
        slk\_Latn & 23.11 & 21.33 & 22.0 & 23.33 & 23.78 & 23.0 & 27.33 & 22.89 \\
        slv\_Latn & 23.78 & 22.56 & 23.0 & 23.44 & 24.67 & 21.56 & 27.33 & 22.89 \\
        sna\_Latn & 23.0 &  & 22.78 & 22.67 & 23.56 & 22.44 & 27.33 & 22.89 \\
        snd\_Arab & 25.33 &  & 22.56 & 22.67 & 23.0 &  & 27.33 & 22.89 \\
        som\_Latn & 22.0 &  & 24.0 & 23.56 & 23.89 &  & 27.33 & 22.89 \\
        sot\_Latn & 23.56 &  & 23.11 & 24.56 & 23.44 & 22.89 & 27.33 & 22.89 \\
        spa\_Latn & 24.44 & 23.22 & 22.67 & 23.78 & 24.33 & 21.56 & 27.33 & 22.89 \\
        srp\_Cyrl & 25.11 & 21.67 & 23.67 & 25.0 & 23.0 & 22.78 & 27.33 & 22.89 \\
        ssw\_Latn & 24.33 &  & 23.44 & 22.78 & 24.22 &  & 27.33 & 22.89 \\
        sun\_Latn & 22.22 & 22.78 & 22.78 & 23.56 & 23.67 & 21.11 & 27.33 & 22.89 \\
        swe\_Latn & 25.56 & 23.33 & 26.44 & 24.0 & 25.56 & 20.44 & 27.33 & 22.89 \\
        swh\_Latn & 26.78 & 22.44 & 26.56 & 23.44 & 23.22 & 21.11 & 27.33 & 22.89 \\
        tam\_Taml & 23.44 &  & 20.89 & 25.78 & 23.44 & 20.44 & 27.33 & 22.89 \\
        tel\_Telu & 24.78 &  & 22.89 & 26.78 & 22.89 & 21.56 & 27.33 & 22.89 \\
        tgk\_Cyrl & 27.56 &  & 23.78 & 23.67 & 23.11 &  & 27.33 & 22.89 \\
        tgl\_Latn & 23.56 &  & 23.11 & 21.89 & 23.44 &  & 27.33 & 22.89 \\
        tha\_Thai & 23.56 & 21.78 & 24.0 & 23.0 & 22.89 & 22.44 & 27.33 & 22.89 \\
        tir\_Ethi & 22.89 &  & 26.11 & 22.0 & 25.44 &  & 27.33 & 22.89 \\
        tsn\_Latn & 24.22 &  & 23.67 & 22.67 & 22.33 &  & 27.33 & 22.89 \\
        tso\_Latn & 23.22 &  & 22.89 & 23.78 & 22.56 &  & 27.33 & 22.89 \\
        tur\_Latn & 23.89 & 22.78 & 23.44 & 23.0 & 23.56 & 20.89 & 27.33 & 22.89 \\
        ukr\_Cyrl & 25.56 &  & 26.33 & 24.89 & 24.78 & 22.67 & 27.33 & 22.89 \\
        urd\_Arab & 25.56 & 22.33 & 22.56 & 24.89 & 22.89 & 21.44 & 27.33 & 22.89 \\
        urd\_Latn & 23.44 &  & 23.44 & 22.78 & 24.11 &  & 27.33 & 22.89 \\
        uzn\_Latn & 23.89 &  & 26.44 & 24.0 & 22.78 &  & 27.33 & 22.89 \\
        vie\_Latn & 24.78 & 22.89 & 24.78 & 24.44 & 21.56 & 22.44 & 27.33 & 22.89 \\
        war\_Latn & 24.56 &  & 24.67 & 22.22 & 23.22 &  & 27.33 & 22.89 \\
        wol\_Latn & 23.67 &  & 25.78 & 21.33 & 23.56 & 20.89 & 27.33 & 22.89 \\
        xho\_Latn & 22.22 &  & 23.67 & 25.22 & 24.22 & 20.67 & 27.33 & 22.89 \\
        yor\_Latn & 22.44 &  & 23.0 & 23.22 & 22.89 &  & 27.33 & 22.89 \\
        zho\_Hans & 22.67 & 21.44 & 23.0 & 23.67 & 23.0 & 21.67 & 27.33 & 22.89 \\
        zho\_Hant & 24.89 & 22.78 & 23.22 & 25.22 & 23.67 & 22.89 & 27.33 & 22.89 \\
        zsm\_Latn & 24.44 & 22.78 & 25.11 & 23.0 & 22.22 & 22.44 & 27.33 & 22.89 \\
        zul\_Latn & 24.33 &  & 23.78 & 22.22 & 24.22 & 23.67 & 27.33 & 22.89 \\
        \bottomrule
    \end{tabular}
    }
\end{table*}

%\end{document}


==> tables/category1_evaluation_tables_index.tex <==
\begin{table*}[ht]
\centering
\caption{Links to category-1 models evaluation results for each task in zero-shot, one-shot, and few-shot setting.}
\label{tab:cat1-eval}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{l l c c c}
\toprule
\textbf{Type} & \textbf{Task} & \textbf{zero-shot} & \textbf{one-shot} & \textbf{few-shot} \\
\midrule
\multirow{5}{*}{Q\&A} 
& \textit{ARC} \cite{clark2018thinksolvedquestionanswering} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_category-1_arc_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_category-1_arc_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_category-1_arc_acc,none.tsv?download=1}{\link} \\ %\midrule
& \textit{MGSM (Direct)} \cite{shi2022languagemodelsmultilingualchainofthought} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_category-1_mgsm_direct_exact_match,flexible-extract.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_category-1_mgsm_direct_exact_match,flexible-extract.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_category-1_mgsm_direct_exact_match,flexible-extract.tsv?download=1}{\link} \\ %\midrule
& \textit{MGSM (Native CoT)} \cite{shi2022languagemodelsmultilingualchainofthought} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_category-1_mgsm_native_cot_exact_match,flexible-extract.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_category-1_mgsm_native_cot_exact_match,flexible-extract.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_category-1_mgsm_native_cot_exact_match,flexible-extract.tsv?download=1}{\link} \\ %\midrule
& \textit{TruthfulQA} \cite{lin-etal-2022-truthfulqa} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_category-1_truthfulqa_mc1_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_category-1_truthfulqa_mc1_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_category-1_truthfulqa_mc1_acc,none.tsv?download=1}{\link} \\ %\midrule
& \textit{MMLU} \cite{hendrycks2021measuringmassivemultitasklanguage} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_category-1_m_mmlu_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_category-1_m_mmlu_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_category-1_m_mmlu_acc,none.tsv?download=1}{\link} \\ \midrule
\multirow{4}{*}{Reasoning} 
& \textit{HellaSwag} \cite{zellers2019hellaswagmachinereallyfinish} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_category-1_hellaswag_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_category-1_hellaswag_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_category-1_hellaswag_acc,none.tsv?download=1}{\link} \\ %\midrule
& \textit{XCOPA} \cite{ponti-etal-2020-xcopa} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_category-1_xcopa_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_category-1_xcopa_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_category-1_xcopa_acc,none.tsv?download=1}{\link} \\ %\midrule
& \textit{XStoryCloze} \cite{lin2022fewshotlearningmultilinguallanguage} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_category-1_xstorycloze_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_category-1_xstorycloze_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_category-1_xstorycloze_acc,none.tsv?download=1}{\link} \\ %\midrule
& \textit{XWinograd} \cite{tikhonov-ryabinin-2021-heads} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_category-1_xwinograd_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_category-1_xwinograd_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_category-1_xwinograd_acc,none.tsv?download=1}{\link} \\ \midrule
\multirow{2}{*}{NLI} 
& \textit{PAWS-X} \cite{pawsx2019emnlp} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_category-1_paws_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_category-1_paws_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_category-1_paws_acc,none.tsv?download=1}{\link} \\ %\midrule
& \textit{XNLI} \cite{conneau2018xnlievaluatingcrosslingualsentence} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_category-1_xnli_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_category-1_xnli_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_category-1_xnli_acc,none.tsv?download=1}{\link} \\ \midrule
\multirow{2}{*}{Reading Comprehension} 
& \textit{LAMBADA} \cite{paperno2016lambadadatasetwordprediction} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_category-1_lambada_openai_mt_stablelm_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_category-1_lambada_openai_mt_stablelm_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_category-1_lambada_openai_mt_stablelm_acc,none.tsv?download=1}{\link} \\ %\midrule
& \textit{Belebele} \cite{bandarkar2023belebele} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_category-1_belebele_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_category-1_belebele_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_category-1_belebele_acc,none.tsv?download=1}{\link} \\ %\midrule
\bottomrule
\end{tabular}
}
\end{table*}

==> tables/category2_evaluation_tables_index.tex <==
\begin{table*}[ht]
\centering
\caption{Links to category-2 models evaluation results for each task in zero-shot, one-shot, and few-shot setting.}
\label{tab:cat2-eval}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{l l c c c}
\toprule
\textbf{Type} & \textbf{Task} & \textbf{zero-shot} & \textbf{one-shot} & \textbf{few-shot} \\
\midrule
\multirow{5}{*}{Q\&A} 
& \textit{ARC} \cite{clark2018thinksolvedquestionanswering} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_category-2_arc_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_category-2_arc_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_category-2_arc_acc,none.tsv?download=1}{\link} \\ %\midrule
& \textit{MGSM (Direct)} \cite{shi2022languagemodelsmultilingualchainofthought} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_category-2_mgsm_direct_exact_match,flexible-extract.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_category-2_mgsm_direct_exact_match,flexible-extract.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_category-2_mgsm_direct_exact_match,flexible-extract.tsv?download=1}{\link} \\ %\midrule
& \textit{MGSM (Native CoT)} \cite{shi2022languagemodelsmultilingualchainofthought} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_category-2_mgsm_native_cot_exact_match,flexible-extract.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_category-2_mgsm_native_cot_exact_match,flexible-extract.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_category-2_mgsm_native_cot_exact_match,flexible-extract.tsv?download=1}{\link} \\ %\midrule
& \textit{TruthfulQA} \cite{lin-etal-2022-truthfulqa} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_category-2_truthfulqa_mc1_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_category-2_truthfulqa_mc1_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_category-2_truthfulqa_mc1_acc,none.tsv?download=1}{\link} \\ %\midrule
& \textit{MMLU} \cite{hendrycks2021measuringmassivemultitasklanguage} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_category-2_m_mmlu_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_category-2_m_mmlu_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_category-2_m_mmlu_acc,none.tsv?download=1}{\link} \\ \midrule
\multirow{4}{*}{Reasoning} 
& \textit{HellaSwag} \cite{zellers2019hellaswagmachinereallyfinish} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_category-2_hellaswag_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_category-2_hellaswag_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_category-2_hellaswag_acc,none.tsv?download=1}{\link} \\ %\midrule
& \textit{XCOPA} \cite{ponti-etal-2020-xcopa} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_category-2_xcopa_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_category-2_xcopa_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_category-2_xcopa_acc,none.tsv?download=1}{\link} \\ %\midrule
& \textit{XStoryCloze} \cite{lin2022fewshotlearningmultilinguallanguage} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_category-2_xstorycloze_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_category-2_xstorycloze_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_category-2_xstorycloze_acc,none.tsv?download=1}{\link} \\ %\midrule
& \textit{XWinograd} \cite{tikhonov-ryabinin-2021-heads} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_category-2_xwinograd_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_category-2_xwinograd_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_category-2_xwinograd_acc,none.tsv?download=1}{\link} \\ \midrule
\multirow{2}{*}{NLI} 
& \textit{PAWS-X} \cite{pawsx2019emnlp} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_category-2_paws_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_category-2_paws_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_category-2_paws_acc,none.tsv?download=1}{\link} \\ %\midrule
& \textit{XNLI} \cite{conneau2018xnlievaluatingcrosslingualsentence} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_category-2_xnli_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_category-2_xnli_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_category-2_xnli_acc,none.tsv?download=1}{\link} \\ \midrule
\multirow{2}{*}{Reading Comprehension} 
& \textit{LAMBADA} \cite{paperno2016lambadadatasetwordprediction} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_category-2_lambada_openai_mt_stablelm_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_category-2_lambada_openai_mt_stablelm_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_category-2_lambada_openai_mt_stablelm_acc,none.tsv?download=1}{\link} \\ %\midrule
& \textit{Belebele} \cite{bandarkar2023belebele} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_category-2_belebele_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_category-2_belebele_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_category-2_belebele_acc,none.tsv?download=1}{\link} \\ %\midrule
\bottomrule
\end{tabular}
}
\end{table*}

==> tables/category3_evaluation_tables_index.tex <==
\begin{table*}[ht]
\centering
\caption{Links to category-3 models evaluation results for each task in zero-shot, one-shot, and few-shot setting.}
\label{tab:cat3-eval}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{l l c c c}
\toprule
\textbf{Type} & \textbf{Task} & \textbf{zero-shot} & \textbf{one-shot} & \textbf{few-shot} \\
\midrule
\multirow{5}{*}{Q\&A} 
& \textit{ARC} \cite{clark2018thinksolvedquestionanswering} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_category-3_arc_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_category-3_arc_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_category-3_arc_acc,none.tsv?download=1}{\link} \\ %\midrule
& \textit{MGSM (Direct)} \cite{shi2022languagemodelsmultilingualchainofthought} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_category-3_mgsm_direct_exact_match,flexible-extract.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_category-3_mgsm_direct_exact_match,flexible-extract.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_category-3_mgsm_direct_exact_match,flexible-extract.tsv?download=1}{\link} \\ %\midrule
& \textit{MGSM (Native CoT)} \cite{shi2022languagemodelsmultilingualchainofthought} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_category-3_mgsm_native_cot_exact_match,flexible-extract.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_category-3_mgsm_native_cot_exact_match,flexible-extract.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_category-3_mgsm_native_cot_exact_match,flexible-extract.tsv?download=1}{\link} \\ %\midrule
& \textit{TruthfulQA} \cite{lin-etal-2022-truthfulqa} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_category-3_truthfulqa_mc1_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_category-3_truthfulqa_mc1_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_category-3_truthfulqa_mc1_acc,none.tsv?download=1}{\link} \\ %\midrule
& \textit{MMLU} \cite{hendrycks2021measuringmassivemultitasklanguage} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_category-3_m_mmlu_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_category-3_m_mmlu_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_category-3_m_mmlu_acc,none.tsv?download=1}{\link} \\ \midrule
\multirow{4}{*}{Reasoning} 
& \textit{HellaSwag} \cite{zellers2019hellaswagmachinereallyfinish} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_category-3_hellaswag_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_category-3_hellaswag_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_category-3_hellaswag_acc,none.tsv?download=1}{\link} \\ %\midrule
& \textit{XCOPA} \cite{ponti-etal-2020-xcopa} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_category-3_xcopa_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_category-3_xcopa_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_category-3_xcopa_acc,none.tsv?download=1}{\link} \\ %\midrule
& \textit{XStoryCloze} \cite{lin2022fewshotlearningmultilinguallanguage} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_category-3_xstorycloze_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_category-3_xstorycloze_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_category-3_xstorycloze_acc,none.tsv?download=1}{\link} \\ %\midrule
& \textit{XWinograd} \cite{tikhonov-ryabinin-2021-heads} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_category-3_xwinograd_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_category-3_xwinograd_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_category-3_xwinograd_acc,none.tsv?download=1}{\link} \\ \midrule
\multirow{2}{*}{NLI} 
& \textit{PAWS-X} \cite{pawsx2019emnlp} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_category-3_paws_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_category-3_paws_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_category-3_paws_acc,none.tsv?download=1}{\link} \\ %\midrule
& \textit{XNLI} \cite{conneau2018xnlievaluatingcrosslingualsentence} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_category-3_xnli_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_category-3_xnli_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_category-3_xnli_acc,none.tsv?download=1}{\link} \\ \midrule
\multirow{2}{*}{Reading Comprehension} 
& \textit{LAMBADA} \cite{paperno2016lambadadatasetwordprediction} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_category-3_lambada_openai_mt_stablelm_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_category-3_lambada_openai_mt_stablelm_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_category-3_lambada_openai_mt_stablelm_acc,none.tsv?download=1}{\link} \\ %\midrule
& \textit{Belebele} \cite{bandarkar2023belebele} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_category-3_belebele_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_category-3_belebele_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_category-3_belebele_acc,none.tsv?download=1}{\link} \\ %\midrule
\bottomrule
\end{tabular}
}
\end{table*}

==> tables/combined_evaluation_tables_index.tex <==
\begin{table*}[ht]
\centering
\caption{Links to combined (all model categories) evaluation results for each task in zero-shot, one-shot, and few-shot setting.}
\label{tab:all-eval}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{l l c c c}
\toprule
\textbf{Type} & \textbf{Task} & \textbf{zero-shot} & \textbf{one-shot} & \textbf{few-shot} \\
\midrule
\multirow{5}{*}{Q\&A} 
& \textit{ARC} \cite{clark2018thinksolvedquestionanswering} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_all_arc_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_all_arc_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_all_arc_acc,none.tsv?download=1}{\link} \\ %\midrule
& \textit{MGSM (Direct)} \cite{shi2022languagemodelsmultilingualchainofthought} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_all_mgsm_direct_exact_match,flexible-extract.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_all_mgsm_direct_exact_match,flexible-extract.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_all_mgsm_direct_exact_match,flexible-extract.tsv?download=1}{\link} \\ %\midrule
& \textit{MGSM (Native CoT)} \cite{shi2022languagemodelsmultilingualchainofthought} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_all_mgsm_native_cot_exact_match,flexible-extract.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_all_mgsm_native_cot_exact_match,flexible-extract.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_all_mgsm_native_cot_exact_match,flexible-extract.tsv?download=1}{\link} \\ %\midrule
& \textit{TruthfulQA} \cite{lin-etal-2022-truthfulqa} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_all_truthfulqa_mc1_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_all_truthfulqa_mc1_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_all_truthfulqa_mc1_acc,none.tsv?download=1}{\link} \\ %\midrule
& \textit{MMLU} \cite{hendrycks2021measuringmassivemultitasklanguage} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_all_m_mmlu_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_all_m_mmlu_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_all_m_mmlu_acc,none.tsv?download=1}{\link} \\ \midrule
\multirow{4}{*}{Reasoning} 
& \textit{HellaSwag} \cite{zellers2019hellaswagmachinereallyfinish} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_all_hellaswag_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_all_hellaswag_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_all_hellaswag_acc,none.tsv?download=1}{\link} \\ %\midrule
& \textit{XCOPA} \cite{ponti-etal-2020-xcopa} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_all_xcopa_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_all_xcopa_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_all_xcopa_acc,none.tsv?download=1}{\link} \\ %\midrule
& \textit{XStoryCloze} \cite{lin2022fewshotlearningmultilinguallanguage} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_all_xstorycloze_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_all_xstorycloze_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_all_xstorycloze_acc,none.tsv?download=1}{\link} \\ %\midrule
& \textit{XWinograd} \cite{tikhonov-ryabinin-2021-heads} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_all_xwinograd_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_all_xwinograd_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_all_xwinograd_acc,none.tsv?download=1}{\link} \\ \midrule
\multirow{2}{*}{NLI} 
& \textit{PAWS-X} \cite{pawsx2019emnlp} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_all_paws_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_all_paws_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_all_paws_acc,none.tsv?download=1}{\link} \\ %\midrule
& \textit{XNLI} \cite{conneau2018xnlievaluatingcrosslingualsentence} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_all_xnli_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_all_xnli_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_all_xnli_acc,none.tsv?download=1}{\link} \\ \midrule
\multirow{2}{*}{Reading Comprehension} 
& \textit{LAMBADA} \cite{paperno2016lambadadatasetwordprediction} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_all_lambada_openai_mt_stablelm_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_all_lambada_openai_mt_stablelm_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_all_lambada_openai_mt_stablelm_acc,none.tsv?download=1}{\link} \\ %\midrule
& \textit{Belebele} \cite{bandarkar2023belebele} & \href{https://zenodo.org/records/13750485/files/evaluation_table_0shot_all_belebele_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750495/files/evaluation_table_1shot_all_belebele_acc,none.tsv?download=1}{\link} & \href{https://zenodo.org/records/13750497/files/evaluation_table_5shot_all_belebele_acc,none.tsv?download=1}{\link} \\ %\midrule
\bottomrule
\end{tabular}
}
\end{table*}

==> tables/hellaswag.tex <==
%\documentclass[11pt, a4paper]{article}
%\usepackage{booktabs}
%\begin{document}

\begin{table*}[htb]
    \centering
    \caption{Hellaswag task}
    \label{tab:hellaswag}
    \resizebox{1.9\columnwidth}{!}{%
    \begin{tabular}{@{}lcccccccc@{}}
    \hline
        \toprule
         Language & lola\_v1 &xlm-roberta-large & mGPT & bloom-1b1 & bloom-1b7 & glot500-base & mbart-large-50 & mt5-large 
         \\
        \midrule
        ar & 31.75 & 24.17 & 28.37 & 29.51 & 31.07 & 24.57 & 26.13 & 25.08 \\
        bn & 26.81 & 0.0 & 26.16 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
        ca & 34.12 & 24.16 & 28.22 & 32.47 & 33.89 & 24.73 & 25.9 & 25.91 \\
        da & 34.83 & 23.69 & 29.88 & 26.45 & 27.23 & 24.52 & 25.65 & 25.17 \\
        de & 37.28 & 24.5 & 30.38 & 27.04 & 27.12 & 25.26 & 26.05 & 25.76 \\
        es & 38.15 & 24.02 & 30.63 & 34.3 & 36.21 & 25.12 & 26.13 & 26.24 \\
        eu & 26.9 & 0.0 & 26.41 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
        fr & 37.62 & 24.23 & 31.02 & 33.58 & 36.15 & 24.95 & 25.72 & 25.71 \\
        gu & 26.77 & 0.0 & 24.4 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
        hi & 29.05 & 24.16 & 27.42 & 28.29 & 28.83 & 24.64 & 26.18 & 25.17 \\
        hr & 28.97 & 24.26 & 27.23 & 27.05 & 26.73 & 24.7 & 26.61 & 24.89 \\
        hu & 31.41 & 24.1 & 28.28 & 26.41 & 26.57 & 24.24 & 25.65 & 25.28 \\
        hy & 26.02 & 23.73 & 25.37 & 25.21 & 25.13 & 23.48 & 24.72 & 23.97 \\
        id & 33.03 & 23.74 & 29.48 & 31.69 & 33.3 & 24.02 & 26.18 & 25.07 \\
        it & 36.31 & 24.21 & 30.27 & 28.2 & 28.65 & 24.78 & 26.31 & 25.53 \\
        kn & 26.02 & 0.0 & 24.92 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
        ml & 25.41 & 0.0 & 25.38 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
        mr & 26.91 & 0.0 & 25.99 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
        ne & 26.59 & 0.0 & 25.79 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
        nl & 35.82 & 0.0 & 30.03 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
        pt & 36.48 & 24.27 & 30.47 & 33.0 & 35.38 & 25.34 & 26.45 & 25.38 \\
        ro & 34.2 & 24.36 & 29.52 & 27.02 & 27.28 & 25.0 & 25.64 & 25.21 \\
        ru & 36.24 & 24.71 & 29.9 & 27.53 & 27.57 & 25.26 & 25.92 & 26.1 \\
        sk & 32.9 & 24.51 & 27.01 & 26.21 & 26.29 & 24.77 & 25.97 & 25.36 \\
        sr & 29.52 & 24.4 & 27.42 & 26.94 & 27.09 & 24.76 & 26.16 & 25.24 \\
        sv & 34.86 & 24.07 & 29.74 & 26.34 & 26.13 & 24.42 & 26.07 & 25.31 \\
        ta & 25.77 & 0.0 & 25.53 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
        te & 25.77 & 0.0 & 25.86 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
        uk & 33.97 & 24.02 & 28.8 & 26.58 & 27.17 & 24.42 & 25.96 & 25.6 \\
        vi & 34.44 & 24.36 & 30.27 & 32.08 & 33.33 & 25.07 & 26.93 & 25.87 \\
        \bottomrule
    \end{tabular}
    }
\end{table*}

%\end{document}


==> tables/lambada.tex <==
%\documentclass[11pt, a4paper]{article}
%\usepackage{booktabs}
%\begin{document}

\begin{table*}[htb]
    \centering
    \caption{Lambada task}
    \label{tab:lambada}
    \resizebox{1.9\columnwidth}{!}{%
    \begin{tabular}{@{}lcccccccc@{}}
    \hline
        \toprule
        Language & lola\_v1 &xlm-roberta-large & mGPT & bloom-1b1 & bloom-1b7 & glot500-base & mbart-large-50 & mt5-large 
         \\
        \midrule
        en & 48.67 & 0.02 & 37.75 & 42.64 & 46.28 & 0.0 & 1.4 & 0.0 \\
        fr & 40.83 & 0.0 & 32.04 & 39.72 & 43.8 & 0.0 & 0.0 & 0.0 \\
        es & 35.8 & 0.23 & 29.63 & 35.84 & 39.26 & 0.0 & 1.77 & 0.0 \\
        de & 54.05 & 0.37 & 40.89 & 13.6 & 17.47 & 0.0 & 0.66 & 0.0 \\
        it & 39.9 & 0.06 & 35.18 & 24.84 & 28.93 & 0.0 & 1.01 & 0.0 \\
        \bottomrule
    \end{tabular}
    }
\end{table*}

%\end{document}


==> tables/m_mmlu.tex <==
%\documentclass[11pt, a4paper]{article}
%\usepackage{booktabs}
%\begin{document}

\begin{table*}[htb]
    \centering
    \caption{M\_mmlu task}
    \label{tab:m_mmlu}
    \resizebox{1.9\columnwidth}{!}{%
    \begin{tabular}{@{}lcccccc@{}}
     \hline
        \toprule
        Language & lola\_v1 & mGPT & bloom-1b1 & bloom-1b7 & mbart-large-50 & mt5-large 
         \\
        \midrule
        ar & 24.13 & 22.87 & 23.78 & 22.9 & 25.48 & 22.72 \\
        bn & 24.22 & 24.13 & 23.99 & 25.56 & 25.31 & 22.62 \\
        ca & 24.69 & 24.1 & 23.34 & 23.4 & 25.55 & 22.64 \\
        da & 23.4 & 23.11 & 23.94 & 24.55 & 25.57 & 22.69 \\
        de & 24.24 & 23.04 & 22.67 & 23.86 & 25.6 & 22.71 \\
        en & 23.51 & 22.85 & 24.07 & 26.04 & 25.6 & 22.71 \\
        es & 24.73 & 22.96 & 23.7 & 25.09 & 25.51 & 22.72 \\
        eu & 24.92 & 23.77 & 22.38 & 24.98 & 25.77 & 22.4 \\
        fr & 24.34 & 24.06 & 23.61 & 23.52 & 25.48 & 22.78 \\
        gu & 24.07 & 23.48 & 23.94 & 22.81 & 25.54 & 22.54 \\
        hi & 24.59 & 24.27 & 23.83 & 23.9 & 25.49 & 22.74 \\
        hr & 23.33 & 22.57 & 23.74 & 24.4 & 25.59 & 22.6 \\
        hu & 24.64 & 22.61 & 24.11 & 23.18 & 25.58 & 22.6 \\
        hy & 23.88 & 23.76 & 24.64 & 24.71 & 25.51 & 22.6 \\
        id & 24.3 & 23.69 & 22.98 & 24.53 & 25.43 & 22.75 \\
        is & 23.16 & 22.97 & 24.36 & 25.09 & 25.6 & 22.71 \\
        it & 24.01 & 22.96 & 23.03 & 23.44 & 25.44 & 22.89 \\
        kn & 23.11 & 24.01 & 24.31 & 24.91 & 25.38 & 22.97 \\
        ml & 23.99 & 22.85 & 24.44 & 24.21 & 25.24 & 22.91 \\
        mr & 25.56 & 23.24 & 23.97 & 24.43 & 25.42 & 22.55 \\
        nb & 23.01 & 22.99 & 23.47 & 24.61 & 25.6 & 22.71 \\
        ne & 23.36 & 24.48 & 23.59 & 24.21 & 25.41 & 22.77 \\
        nl & 23.84 & 23.09 & 23.87 & 23.9 & 25.62 & 22.8 \\
        pt & 23.83 & 22.88 & 22.85 & 25.11 & 25.47 & 22.83 \\
        ro & 24.52 & 22.89 & 23.54 & 23.32 & 25.45 & 22.66 \\
        ru & 23.49 & 23.25 & 23.11 & 25.42 & 25.42 & 22.7 \\
        sk & 23.49 & 22.86 & 24.31 & 24.04 & 25.56 & 22.71 \\
        sr & 23.46 & 22.85 & 23.91 & 24.39 & 25.57 & 22.74 \\
        sv & 23.86 & 22.92 & 24.26 & 24.16 & 25.5 & 22.76 \\
        ta & 23.2 & 23.5 & 24.64 & 24.55 & 25.59 & 22.73 \\
        te & 24.41 & 23.02 & 24.57 & 23.33 & 25.3 & 22.94 \\
        uk & 24.1 & 24.35 & 23.32 & 24.77 & 25.37 & 22.69 \\
        vi & 24.71 & 23.87 & 23.17 & 23.9 & 25.56 & 22.77 \\
        zh & 24.43 & 22.84 & 24.22 & 24.12 & 25.47 & 22.77 \\
        \bottomrule
    \end{tabular}
    
    }
\end{table*}

%\end{document}


==> tables/mgsm_direct.tex <==
%\documentclass[11pt, a4paper]{article}
%\usepackage{booktabs}
%\begin{document}

\begin{table*}[htb]
    \centering
    \caption{mgsm\_direct task}
    \label{tab:mgsm_direct}
    \resizebox{1.9\columnwidth}{!}{%
    \begin{tabular}{@{}lcccccccc@{}}
    \hline
        \toprule
        Language & lola\_v1 & xlm-roberta-large & mGPT & bloom-1b1 & bloom-1b7 & glot500-base & mbart-large-50 & mt5-large 
        \\
        \midrule
        bn & 0.0 & 0.0 & 2.0 & 2.8 & 1.6 & 0.0 & 0.0 & 0.4 \\
        de & 0.8 & 0.0 & 2.4 & 1.6 & 1.6 & 0.0 & 0.0 & 0.8 \\
        en & 0.4 & 0.0 & 2.4 & 2.4 & 2.0 & 0.0 & 0.4 & 0.8 \\
        es & 1.2 & 0.0 & 1.6 & 1.2 & 2.4 & 0.0 & 0.0 & 0.0 \\
        fr & 0.8 & 0.0 & 2.4 & 1.6 & 2.0 & 0.0 & 0.0 & 1.2 \\
        ja & 0.8 & 0.0 & 1.2 & 2.8 & 2.0 & 0.0 & 0.4 & 0.4 \\
        ru & 0.8 & 0.0 & 2.4 & 1.2 & 2.0 & 0.0 & 0.0 & 0.8 \\
        sw & 1.2 & 0.0 & 1.6 & 1.6 & 1.6 & 0.0 & 0.0 & 0.8 \\
        te & 0.0 & 0.0 & 2.0 & 1.2 & 3.2 & 0.0 & 0.0 & 0.0 \\
        th & 0.4 & 0.0 & 0.8 & 2.0 & 2.8 & 0.0 & 0.4 & 0.4 \\
        zh & 0.0 & 0.0 & 2.4 & 2.4 & 1.6 & 0.0 & 0.0 & 0.4 \\
        \bottomrule
    \end{tabular}
    }
\end{table*}

%\end{document}


==> tables/mgsm_native.tex <==
%\documentclass[11pt, a4paper]{article}
%\usepackage{booktabs}
%\begin{document}

\begin{table*}[htb]
    \centering
    \caption{mgsm\_native task}
    \label{tab:mgsm_native}
    \resizebox{1.9\columnwidth}{!}{%
    \begin{tabular}{@{}lcccccccc@{}}
    \hline
        \toprule
         Language & lola\_v1 & xlm-roberta-large & mGPT & bloom-1b1 & bloom-1b7 & glot500-base & mbart-large-50 & mt5-large 
         \\
        \midrule
        bn & 0.4 & 0.0 & 2.0 & 1.6 & 0.8 & 0.0 & 0.0 & 0.4 \\
        de & 1.2 & 0.0 & 2.0 & 0.8 & 0.4 & 0.0 & 0.0 & 0.8 \\
        en & 0.4 & 0.0 & 2.8 & 2.0 & 2.4 & 0.0 & 0.4 & 0.4 \\
        es & 1.2 & 0.0 & 2.4 & 1.6 & 1.2 & 0.0 & 0.0 & 0.0 \\
        fr & 0.4 & 0.0 & 1.2 & 2.0 & 1.6 & 0.0 & 0.0 & 0.8 \\
        ja & 0.4 & 0.0 & 0.8 & 1.6 & 2.0 & 0.0 & 0.0 & 0.0 \\
        ru & 1.2 & 0.0 & 1.2 & 1.2 & 0.0 & 0.0 & 0.0 & 2.0 \\
        sw & 0.4 & 0.0 & 0.8 & 0.8 & 0.8 & 0.0 & 0.0 & 0.4 \\
        te & 0.4 & 0.0 & 0.4 & 1.6 & 2.0 & 0.0 & 0.0 & 0.8 \\
        th & 0.4 & 0.0 & 3.2 & 1.6 & 2.0 & 0.0 & 0.4 & 1.2 \\
        zh & 1.2 & 0.0 & 3.2 & 2.0 & 2.0 & 0.0 & 0.0 & 0.0 \\
        \bottomrule
    \end{tabular}
    }
\end{table*}

%\end{document}


==> tables/name.tex <==
\begin{table*}[t!]
 \small
 
 % \vspace{-4mm}
  \label{tab:languages}
 \begin{center}
  \begin{tabular}{@{}llllllllc@{}}
    \toprule
    &&\textbf{Tasks} & \textbf{\# Language} & \textbf{NLP task} & \textbf{Metric} \\
    \midrule
   % &\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Medium}}}
   % \midrule
    %&\parbox[t]{2mm}{\multirow{12}{*}{\rotatebox[origin=c]{90}{Low}}}
    && arc & 31 & Questions Answering & Acc \\
    && hellaswag & 31 & Commonsense NLI & Acc  \\
    && lambada\_openai\_mt & 5 & Language Modeling & Acc \\
    && m\_mmlu & 34 & Reading Comprehension & Acc   \\
    && mgsm\_direct & 11 & Question Answering  & Exact_match  \\
    && mgsm\_native & 11 & Question Answering & Exact_match\\
    && paws & 7 & NLI & Acc\\
    && truthfilqa\_mc1 & Question Answering & Acc  \\
    && xcopa & 11 & Causal Commonsense Reasoning & Acc   \\
    && xnli & 15 & NLI & Acc  \\
    && xstorycloze & 11 & Commonsense Reasoning & Acc  \\
    && xwinograd & 6 & Commonsense Reasoning & Acc
      \caption{We provide the evaluation tasks used to evaluate LOLA, the number of languages covered by each task with their corresponding metrics.}
  \end{tabular}
 % }
  %\vspace{-3mm}
  \end{center}
\end{table*}

==> tables/paws.tex <==
%\documentclass[11pt, a4paper]{article}
%\usepackage{booktabs}
%\begin{document}

\begin{table*}[htb]
    \centering
    \caption{paws task}
    \label{tab:paws}
    \resizebox{1.9\columnwidth}{!}{%
    \begin{tabular}{@{}lcccccccc@{}}
    \hline
        \toprule
         Language & lola\_v1 & xlm-roberta-large & mGPT & bloom-1b1 & bloom-1b7 & glot500-base & mbart-large-50 & mt5-large 
         \\
        \midrule
        de & 52.65 & 55.15 & 49.25 & 53.45 & 50.3 & 52.35 & 51.0 & 51.05 \\
        en & 45.25 & 49.6 & 43.6 & 49.1 & 52.8 & 48.8 & 48.95 & 47.35 \\
        es & 49.95 & 45.35 & 48.15 & 50.55 & 49.6 & 51.35 & 46.25 & 49.35 \\
        fr & 54.75 & 49.6 & 54.8 & 54.75 & 54.75 & 45.9 & 46.85 & 47.3 \\
        ja & 55.35 & 52.5 & 54.85 & 51.2 & 56.5 & 51.25 & 55.85 & 51.45 \\
        ko & 54.15 & 52.75 & 52.5 & 50.25 & 54.4 & 53.45 & 53.25 & 48.55 \\
        zh & 52.85 & 52.05 & 51.6 & 51.0 & 54.75 & 50.65 & 55.4 & 47.85 \\
        \bottomrule
        \hline
    \end{tabular}
    }
\end{table*}

%\end{document}


==> tables/truthfulqa.tex <==
%\documentclass[11pt, a4paper]{article}
%\usepackage{booktabs}
%\begin{document}

\begin{table*}[htb]
    \centering
    \caption{Truthfulqa task}
    \label{tab:truthfulqa}
    \resizebox{1.9\columnwidth}{!}{%
    \begin{tabular}{@{}lcccccccc@{}}
     \hline
        \toprule
        Language & lola\_v1 & xlm-roberta-large & mGPT & bloom-1b1 & bloom-1b7 & glot500-base & mbart-large-50 & mt5-large 
         \\
        \midrule
        ar & 26.26 & 24.97 & 28.98 & 28.33 & 28.72 & 24.97 & 27.04 & 25.74 \\
        bn & 26.12 & 23.69 & 26.12 & 25.1 & 24.97 & 25.1 & 25.35 & 24.71 \\
        ca & 22.27 & 24.58 & 22.01 & 25.61 & 28.06 & 24.58 & 22.78 & 21.62 \\
        da & 25.35 & 21.51 & 27.66 & 21.51 & 22.92 & 21.77 & 22.15 & 23.94 \\
        de & 23.98 & 22.84 & 24.49 & 24.87 & 25.13 & 22.97 & 26.65 & 22.84 \\
        es & 21.17 & 23.83 & 25.73 & 25.86 & 26.24 & 24.84 & 24.21 & 22.81 \\
        eu & 24.29 & 23.9 & 25.71 & 24.55 & 24.81 & 22.74 & 23.64 & 24.94 \\
        fr & 22.74 & 22.62 & 24.9 & 25.29 & 26.43 & 23.63 & 23.25 & 22.62 \\
        gu & 27.77 & 26.81 & 25.44 & 26.13 & 27.22 & 27.77 & 27.22 & 25.85 \\
        hi & 24.06 & 26.13 & 25.49 & 24.45 & 27.04 & 25.49 & 22.64 & 24.32 \\
        hr & 26.53 & 22.37 & 26.79 & 23.93 & 25.88 & 23.28 & 24.84 & 22.63 \\
        hu & 26.59 & 24.25 & 29.05 & 27.11 & 27.37 & 24.9 & 24.25 & 20.88 \\
        hy & 26.76 & 29.11 & 27.12 & 25.86 & 27.67 & 30.56 & 29.84 & 26.76 \\
        id & 25.58 & 24.29 & 25.96 & 26.35 & 28.41 & 22.75 & 25.84 & 23.26 \\
        it & 23.63 & 23.88 & 28.1 & 25.29 & 25.42 & 22.86 & 25.93 & 22.09 \\
        kn & 28.02 & 29.06 & 28.47 & 28.61 & 28.17 & 28.02 & 29.06 & 28.61 \\
        ml & 29.83 & 28.96 & 28.82 & 26.22 & 28.39 & 28.39 & 29.25 & 27.09 \\
        mr & 27.23 & 26.18 & 27.88 & 26.57 & 28.01 & 24.48 & 25.13 & 25.39 \\
        ne & 26.74 & 27.39 & 23.77 & 26.61 & 27.91 & 26.61 & 27.26 & 26.49 \\
        nl & 24.71 & 23.57 & 24.84 & 22.29 & 23.82 & 25.1 & 26.88 & 22.68 \\
        pt & 21.45 & 24.62 & 26.52 & 24.62 & 25.89 & 24.49 & 27.03 & 23.98 \\
        ro & 24.01 & 23.36 & 25.55 & 21.57 & 22.98 & 21.82 & 22.59 & 23.62 \\
        ru & 24.49 & 24.75 & 24.75 & 30.08 & 30.84 & 24.11 & 29.7 & 23.73 \\
        sk & 23.91 & 21.34 & 22.37 & 20.18 & 21.08 & 23.01 & 22.62 & 24.42 \\
        sr & 26.24 & 24.71 & 25.86 & 26.75 & 27.77 & 22.42 & 25.86 & 22.93 \\
        sv & 24.42 & 24.68 & 25.58 & 23.39 & 23.0 & 24.81 & 25.32 & 25.06 \\
        ta & 27.73 & 27.46 & 26.51 & 26.65 & 26.78 & 27.86 & 27.86 & 26.24 \\
        te & 27.23 & 29.5 & 25.82 & 25.53 & 26.52 & 28.79 & 27.66 & 26.52 \\
        uk & 25.19 & 23.51 & 26.75 & 26.88 & 30.13 & 22.99 & 26.62 & 24.03 \\
        vi & 26.88 & 21.53 & 28.92 & 25.22 & 29.94 & 20.64 & 26.37 & 22.42 \\
        zh & 22.34 & 24.24 & 24.62 & 22.72 & 23.98 & 24.37 & 25.13 & 25.63 \\
        \bottomrule
    \end{tabular}
    }
\end{table*}

%\end{document}


==> tables/xcopa.tex <==
%\documentclass[11pt, a4paper]{article}
%\usepackage{booktabs}
%\begin{document}

\begin{table*}[htb]
    \centering
    \caption{xcopa task}
    \label{tab:xcopa}
   \resizebox{1.9\columnwidth}{!}{%
    \begin{tabular}{@{}lcccccccc@{}}
     \hline
        \toprule
       Language & lola\_v1 & xlm-roberta-large & mGPT & bloom-1b1 & bloom-1b7 & glot500-base & mbart-large-50 & mt5-large
         \\
        \midrule
        et & 53.8 & 50.6 & 53.0 & 50.4 & 47.4 & 47.2 & 51.2 & 54.6 \\
        ht & 50.4 & 52.2 & 49.8 & 53.0 & 50.2 & 54.2 & 53.0 & 49.0 \\
        id & 63.0 & 50.8 & 58.8 & 64.8 & 63.0 & 51.0 & 51.8 & 53.8 \\
        it & 63.0 & 49.8 & 58.2 & 50.8 & 52.6 & 48.8 & 48.6 & 50.8 \\
        qu & 50.6 & 51.8 & 50.6 & 51.2 & 50.6 & 47.2 & 50.8 & 52.4 \\
        sw & 54.0 & 54.6 & 56.4 & 54.6 & 51.8 & 54.2 & 54.4 & 54.2 \\
        ta & 54.8 & 53.2 & 53.2 & 57.0 & 56.4 & 55.6 & 54.8 & 55.6 \\
        th & 54.4 & 52.2 & 55.2 & 53.2 & 53.2 & 50.4 & 57.2 & 53.2 \\
        tr & 55.2 & 53.4 & 56.0 & 52.8 & 52.8 & 56.0 & 54.2 & 57.4 \\
        vi & 65.2 & 47.0 & 60.2 & 62.4 & 65.8 & 49.8 & 52.2 & 53.0 \\
        zh & 56.6 & 52.4 & 54.0 & 59.4 & 61.4 & 50.2 & 54.4 & 52.4 \\
        \bottomrule
    \end{tabular}
    }
\end{table*}

%\end{document}


==> tables/xnli.tex <==
%\documentclass[11pt, a4paper]{article}
%\usepackage{booktabs}
%\begin{document}

\begin{table*}[htb]
    \centering
    \caption{xnli task}
    \label{tab:xnli}
   \resizebox{1.9\columnwidth}{!}{%
    \begin{tabular}{@{}lcccccccc@{}}
     \hline
        \toprule
       Language & lola\_v1 & xlm-roberta-large & mGPT & bloom-1b1 & bloom-1b7 & glot500-base & mbart-large-50 & mt5-large
         \\
        \midrule
        ar & 33.33 & 33.45 & 33.82 & 33.17 & 33.82 & 33.33 & 34.3 & 33.86 \\
        bg & 44.3 & 31.16 & 41.73 & 35.18 & 36.47 & 30.52 & 35.42 & 34.62 \\
        de & 45.18 & 31.49 & 44.78 & 38.19 & 39.08 & 32.81 & 35.74 & 33.17 \\
        el & 42.09 & 33.21 & 35.42 & 33.73 & 33.94 & 31.81 & 33.37 & 33.53 \\
        en & 52.05 & 27.03 & 49.36 & 51.16 & 51.12 & 30.36 & 37.23 & 34.02 \\
        es & 45.82 & 30.36 & 42.81 & 47.15 & 47.63 & 32.73 & 33.33 & 33.94 \\
        fr & 46.63 & 26.31 & 44.06 & 46.47 & 46.67 & 32.49 & 36.22 & 32.37 \\
        hi & 38.03 & 33.29 & 41.33 & 42.57 & 42.89 & 33.09 & 35.26 & 32.77 \\
        ru & 46.63 & 30.88 & 43.21 & 40.08 & 39.96 & 33.33 & 36.87 & 33.9 \\
        sw & 33.25 & 33.69 & 41.89 & 34.34 & 34.34 & 33.29 & 31.41 & 33.57 \\
        th & 39.52 & 34.62 & 35.78 & 33.45 & 33.53 & 33.05 & 33.98 & 32.61 \\
        tr & 42.41 & 33.94 & 40.12 & 35.22 & 35.34 & 33.94 & 39.2 & 32.81 \\
        ur & 33.86 & 33.69 & 34.22 & 37.11 & 38.23 & 33.82 & 33.37 & 33.21 \\
        vi & 39.6 & 31.89 & 45.5 & 41.89 & 44.46 & 33.49 & 34.38 & 34.62 \\
        zh & 35.3 & 33.69 & 33.61 & 36.55 & 35.34 & 33.65 & 33.33 & 32.81 \\
        \bottomrule
    \end{tabular}
    }
\end{table*}

%\end{document}


==> tables/xstorycloze.tex <==
%\documentclass[11pt, a4paper]{article}
%\usepackage{booktabs}
%\begin{document}

\begin{table*}[htb]
    \centering
    \caption{xstorycloze task}
    \label{tab:xstorycloze}
     \resizebox{1.9\columnwidth}{!}{%
    \begin{tabular}{@{}lcccccccc@{}}
     \hline
        \toprule
       Language & lola\_v1 & xlm-roberta-large & mGPT & bloom-1b1 & bloom-1b7 & glot500-base & mbart-large-50 & mt5-large
         \\
        \midrule
        ar & 54.07 & 47.25 & 49.31 & 52.88 & 55.0 & 48.71 & 49.7 & 47.32 \\
        en & 67.7 & 49.17 & 59.96 & 62.54 & 64.39 & 46.53 & 50.43 & 50.43 \\
        es & 62.87 & 45.6 & 55.46 & 58.31 & 60.82 & 47.05 & 49.9 & 49.77 \\
        eu & 55.0 & 47.19 & 54.6 & 54.33 & 54.93 & 47.72 & 49.31 & 49.7 \\
        hi & 55.99 & 48.11 & 52.75 & 55.59 & 56.85 & 48.18 & 52.28 & 48.31 \\
        id & 58.31 & 46.26 & 53.14 & 57.78 & 59.83 & 44.21 & 49.37 & 47.52 \\
        my & 50.1 & 47.65 & 51.22 & 46.26 & 47.12 & 47.12 & 47.52 & 49.04 \\
        ru & 62.48 & 47.85 & 56.65 & 48.25 & 50.36 & 46.19 & 48.71 & 47.85 \\
        sw & 53.08 & 47.25 & 55.0 & 50.43 & 52.28 & 46.86 & 49.64 & 49.24 \\
        te & 56.98 & 50.17 & 57.25 & 56.32 & 56.52 & 49.77 & 52.08 & 50.1 \\
        zh & 56.19 & 47.65 & 53.41 & 58.04 & 58.31 & 46.26 & 49.77 & 47.12 \\
        \bottomrule
    \end{tabular}
    }
\end{table*}

%\end{document}


==> tables/xwinograd.tex <==
%\documentclass[11pt, a4paper]{article}
%\usepackage{booktabs}
%\begin{document}

\begin{table*}[htb]
    \centering
    \caption{xwinograd task}
    \label{tab:xwinograd}
     \resizebox{1.9\columnwidth}{!}{%
    \begin{tabular}{@{}lcccccccc@{}}
     \hline
        \toprule
       Language & lola\_v1 & xlm-roberta-large & mGPT & bloom-1b1 & bloom-1b7 & glot500-base & mbart-large-50 & mt5-large
         \\
        \midrule
        en & 75.01 & 47.66 & 62.67 & 69.94 & 74.54 & 47.61 & 50.41 & 54.54 \\
        fr & 60.24 & 40.96 & 59.04 & 66.27 & 68.67 & 44.58 & 42.17 & 55.42 \\
        ja & 61.11 & 45.78 & 53.49 & 52.87 & 54.22 & 47.86 & 51.41 & 53.39 \\
        pt & 62.74 & 46.77 & 57.41 & 63.88 & 63.5 & 50.57 & 49.05 & 51.71 \\
        ru & 59.37 & 46.98 & 58.1 & 54.29 & 52.38 & 44.76 & 52.06 & 51.75 \\
        zh & 66.47 & 44.84 & 67.46 & 69.05 & 69.64 & 43.85 & 49.8 & 47.22 \\
        \bottomrule
    \end{tabular}
    }
\end{table*}

%\end{document}

